On the Permanence of Vertices in Network Communities

Despite the prevalence of community detection algorithms, relatively less work has been done on understanding whether a network is indeed modular and how resilient the community structure is under perturbations. To address this issue, we propose a new vertex-based metric called "permanence", that can quantitatively give an estimate of the community-like structure of the network. The central idea of permanence is based on the observation that the strength of membership of a vertex to a community depends upon the following two factors: (i) the distribution of external connectivity of the vertex to individual communities and not the total external connectivity, and (ii) the strength of its internal connectivity and not just the total internal edges. In this paper, we demonstrate that compared to other metrics, permanence provides (i) a more accurate estimate of a derived community structure to the ground-truth community and (ii) is more sensitive to perturbations in the network. As a by-product of this study, we have also developed a community detection algorithm based on maximizing permanence. For a modular network structure, the results of our algorithm match well with ground-truth communities.

==> conclusion.tex <==
\vspace{-0.6cm}
\section{Conclusion}
In this paper, we proposed a novel vertex-level metric, called {\em permanence}, which is able to reduce many of the shortcomings of modularity.
We
demonstrated with
analytical proofs and experiments on synthetic and real-world networks that permanence is an effective community evaluation metric compared to other well-known approaches such as modularity, conductance and cut-ratio. We further observed that permanence is tolerant to random fluctuations up to a certain threshold, after which it degrades sharply. Finally, we  showed how using
permanence as an optimization metric yields efficient and more realistic community structures from different networks. 

The proposed metric calls for deeper levels of investigation. To prove the robustness of our proposed metric, networks from diverse
areas have to be tested. We also plan to extend permanence metric to enable evaluation of
the quality of overlapping community structures and to weighted and directed networks. With the
gradual increase of network size in time-varying environment, we are interested to see how permanence captures the movement of a vertex in
different communities. Overall, we believe that this metric will help in formulating a strong theoretical foundation in the identification and evaluation of various types of community strictures where the ground-truth is not known. 
